ELVES-Dwarf. II. A Systematic Search for Satellite Systems of Dwarf Galaxies in the Local Volume

We present the Exploration of Local VolumE Satellites of Dwarf Galaxies (ELVES-Dwarf) survey, a systematic census of satellite systems around dwarf hosts in the Local Volume. Our final sample comprises 39 predominantly isolated hosts with stellar masses $10^{7}<M_\star<10^{10}\,M_\odot$, including 32 hosts searched uniformly in this work and 7 drawn from the literature. We search for satellite candidates within the projected virial radius of each host using $155~\mathrm{deg}^2$ of Legacy Surveys imaging data. We determine satellite membership using surface brightness fluctuation distances from Subaru/HSC, Magellan/IMACS, and Gemini/GMOS imaging, supplemented by literature TRGB distances and radial velocities. From 207 candidates, we confirm 39 satellites with $M_\star>10^5\,M_\odot$ around the 39 hosts. Above our fiducial completeness threshold of $M_\star\gtrsim10^{5.7}\,M_\odot$ and within the projected virial radius, 21 hosts have no confirmed satellites, 10 have one, six have two, and two have four, revealing substantial host-to-host scatter in satellite abundance. Overall, the observed satellite abundances and stellar mass functions are broadly consistent with predictions from the cosmological simulation TNG50 and galaxy formation models calibrated using Milky Way satellites. The projected radial distribution of the satellites is also consistent with theoretical expectations and with satellite populations around Milky Way-mass hosts. In contrast, the quenched fraction of satellites around dwarf hosts is substantially lower than around Milky Way-mass hosts, suggesting that environmental quenching is less efficient in dwarf halos. ELVES-Dwarf provides the first large, homogeneous, distance-confirmed sample of satellites around dwarf hosts and establishes a foundation for understanding galaxy formation and evolution in less-dense environments.

==> tables/literature_hosts.tex <==
% \begin{longrotatetable}
% \begin{deluxetable*}{lLLCCCCCCCcp{4.5cm}}
% \tablecaption{Classical Satellites of Dwarf Galaxies in Literature \label{tab:literature}}
% \tablewidth{0pt}
% \tablehead{
% \colhead{Name} & \colhead{R.A.} & \colhead{Decl.} & \colhead{Distance} & \colhead{$M_V$} & 
% \colhead{$\log M_{\star}$} & \colhead{$r_{\rm eff}$} & \colhead{$\Theta_1$} & \colhead{$\Theta_5$} & \colhead{$\Theta_j$} & \colhead{Conf.} & \colhead{Ref.} \\
% \colhead{} & \colhead{(deg)} & \colhead{(deg)} & \colhead{(Mpc)} & \colhead{(mag)} & 
% \colhead{$M_\odot$} & \colhead{(kpc)} & \colhead{} & \colhead{} & \colhead{} & \colhead{} & \colhead{}
% }
% \startdata
% LMC & 80.8942 & -69.7561 & 0.05 & -18.1 & 9.3 & \nodata & 3.5 & 3.6 & 1.7 & \nodata & \citet{Skibba2012LMC} \\
% \hspace{1em}SMC & 13.1580 & -72.8003 & 0.06 & -16.8 & 8.5 & 1.08 & \nodata & \nodata & \nodata & Y & \citet{Pace2024} \\
% \hline
% M33 & 23.4617 & 30.6603 & 0.84 & -18.8 & 9.7 & \nodata & 1.5 & 1.5 & 1.7 & \nodata & \citet{Corbelli2014} \\
% \hspace{1em} No Satellites \\
% \hline
% NGC~6822 & 296.2404 & -14.8031 & 0.46 & -15.2 & 8.1 & \nodata & 0.5 & 0.6 & 1.7 & \nodata & \citet{Zhang2021_NGC6822} \\
% \hspace{1em} No Satellites \\
% \hline
% NGC~3109 & 150.7769 & -26.1549 & 1.34 & -14.9 & 8.2 & \nodata & -0.3 & -0.1 & -1.2 & \nodata & \citetalias{McConnachie2012} \\
% \hspace{1em}Antlia & 151.0171 & -27.3311 & 1.35 & -10.4 & 6.4 & 0.46 & \nodata & \nodata & \nodata & Y & \citetalias{McConnachie2012} \\
% \hspace{1em}Antlia B & 147.2337 & -25.9900 & 1.29 & -9.7 & 6.2 & 0.27 & \nodata & \nodata & \nodata & Y & \citet{Sand2015} \\
% \hline
% NGC~55 & 3.7208 & -39.1966 & 2.34 & -18.5 & 9.7 & \nodata & 0.0 & 0.2 & 0.2 & \nodata & \citetalias{McConnachie2012} \\
% \hspace{1em}NGC55-dw1 & 3.8740 & -38.4190 & 2.20 & -8.0 & 5.2 & 2.20 & \nodata & \nodata & \nodata & Y & \citet{McNanna2024} \\
% \hline
% NGC~2403 & 114.2117 & 65.6022 & 3.19 & -20.5 & 9.7 & \nodata & 0.2 & 0.6 & 1.9 & \nodata & \citet{Karachentsev2004} \\
% \hspace{1em}MADCASH-1 & 114.2140 & 65.6010 & 3.41 & -7.8 & 5.3 & 0.18 & \nodata & \nodata & \nodata & Y & \citet{Carlin2016,Carlin2024} \\
% \hspace{1em}DDO044 & 113.5479 & 66.8797 & 2.96 & -12.9 & 7.3 & 0.74 & \nodata & \nodata & \nodata & Y & \citet{Karachentsev1999DDO044,Carlin2019} \\
% \hline
% NGC~4214 & 183.9121 & 36.3275 & 3.04 & -17.5 & 8.8 & \nodata & 0.6 & 0.8 & -0.6 & \nodata & \citet{Dalcanton2009} \\
% \hspace{1em}MADCASH-2 & 182.5281 & 35.4429 & 3.00 & -9.2 & 5.8 & 0.13 & \nodata & \nodata & \nodata & Y & \citet{Carlin2021} \\
% \hspace{1em}DDO113 & 183.7412 & 36.2189 & 2.95 & -12.2 & 7.1 & 0.62 & \nodata & \nodata & \nodata & Y & \citet{Garling2020} \\
% \hline
% NGC~4449 & 187.0458 & 44.0936 & 4.02 & -18.4 & 9.5 & \nodata & 0.8 & 0.8 & 1.4 & \nodata & \citet{Sabbi2018} \\
% \hspace{1em}LV J1228+4358 & 187.1867 & 43.9683 & 4.07 & -13.0 & 7.0 & 1.30 & \nodata & \nodata & \nodata & Y & \citet{Martinez-Delgado2012,Garling2021} \\
% \hline
% NGC~5023 & 198.0496 & 44.0386 & 6.05 & -16.5 & 8.8 & \nodata & -0.9 & -0.3 & -1.1 & \nodata & \citetalias{Karachentsev2013} \\
% \hspace{1em}dw1310+4358 & 197.7499 & 43.9802 & \nodata & -8.0 & 5.7 & 0.12 & \nodata & \nodata & \nodata & N & \citet{Carlsten2020} \\
% \hspace{1em}dw1314+4420 & 198.6433 & 44.3342 & \nodata & -7.0 & 5.0 & 0.10 & \nodata & \nodata & \nodata & N & \citet{Carlsten2020} \\
% \hline
% NGC~1156 & 44.9267 & 25.2375 & 6.87 & -17.4 & 9.0 & \nodata & -1.5 & -1.2 & -1.3 & \nodata & \citetalias{Karachentsev2013} \\
% \hspace{1em}NGC1156-dw1 & 45.0758 & 25.2489 & \nodata & -10.5 & 6.1 & \nodata & \nodata & \nodata & \nodata & N & \citetalias{Karachentsev2013} \\
% \hspace{1em}NGC1156-dw2 & 45.1138 & 25.3051 & \nodata & -10.1 & 6.3 & \nodata & \nodata & \nodata & \nodata & N & \citetalias{Karachentsev2013} \\
% \hspace{1em}dw0301+2446 & 45.3842 & 24.7832 & \nodata & -10.6 & 6.5 & \nodata & \nodata & \nodata & \nodata & N & \citet{Carlsten2020} \\
% \hspace{1em}AGES J030039+254656 & 45.1625 & 25.7822 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & N & \citet{Minchin2010} \\
% \hline
% NGC~45 & 3.5162 & -23.1822 & 6.64 & -20.0 & 9.1 & \nodata & -1.0 & -0.9 & 0.2 & \nodata & \citet{Muller2020} \\
% \hspace{1em} No Satellites \\
% \hline
% NGC~24 & 2.4850 & -24.9633 & 7.31 & -20.3 & 9.2 & \nodata & 0.3 & 0.6 & 0.1 & \nodata & \citetalias{Karachentsev2013} \\
% \hspace{1em}dw0009-25 & 2.4075 & -25.0492 & \nodata & -8.3 & 5.9 & 0.28 & \nodata & \nodata & \nodata & N & \citet{Muller2020} \\
% \hspace{1em}dw0010-25 & 2.6592 & -25.3349 & \nodata & -11.6 & 6.7 & 1.05 & \nodata & \nodata & \nodata & N & \citet{Muller2020} \\
% \hline
% NGC~672 & 26.9717 & 27.4336 & 7.18 & -18.2 & 9.4 & \nodata & 0.2 & 0.3 & 0.2 & \nodata & \citetalias{Karachentsev2013} \\
% \hspace{1em}IC1727 & 26.8745 & 27.3333 & 7.45 & -17.3 & 9.2 & 3.30 & \nodata & \nodata & \nodata & Y & \citetalias{Karachentsev2013} \\
% \hspace{1em}NGC672-dwA & 26.8304 & 27.2548 & \nodata & -9.4 & 5.5 & 0.20 & \nodata & \nodata & \nodata & N & \citet{Davis2024} \\
% \hline
% NGC~925 & 36.8167 & 33.5781 & 9.55 & -19.8 & 9.9 & \nodata & 1.0 & 1.1 & 0.5 & \nodata & \citetalias{Karachentsev2013} \\
% \hspace{1em}d0226+3325 & 36.7200 & 33.4269 & \nodata & -12.0 & 7.0 & 1.50 & \nodata & \nodata & \nodata & N & \citet{PWE98,Davis2024} \\
% \hline
% M96-DF6 & 161.7212 & 12.7426 & 10.20 & -13.4 & 7.6 & \nodata & 2.0 & 2.0 & 2.0 & \nodata & \citet{Cohen2018} \\
% \hspace{1em}dw1046+1244 & 161.6915 & 12.7499 & \nodata & -8.1 & 5.4 & 0.21 & \nodata & \nodata & \nodata & N & \citet{Muller2023} \\
% \hline
% \enddata
% \tablecomments{Hosts in the ELVES survey \citep{CarlstenELVES2022}, such as NGC628, are not included in this table.}
% \end{deluxetable*}
% \end{longrotatetable}

\setlength{\tabcolsep}{4pt}
\begin{longrotatetable}
\begin{deluxetable*}{lLLCCCCCCCcp{4cm}}
\tabletypesize{\footnotesize}
\tablecaption{Classical Satellites of Dwarf Galaxies from the Literature \label{tab:literature}}
\tablewidth{0pt}
\tablehead{
\colhead{Name} & \colhead{R.A.} & \colhead{Decl.} & \colhead{Distance} & \colhead{$M_V$} & 
\colhead{$\log M_{\star}$} & \colhead{$r_{\rm eff}$} & \colhead{$\Theta_1$} & \colhead{$\Theta_5$} & \colhead{$\Theta_j$} & \colhead{Conf.} & \colhead{Ref.} \\
\colhead{} & \colhead{(deg)} & \colhead{(deg)} & \colhead{(Mpc)} & \colhead{(mag)} & 
\colhead{$M_\odot$} & \colhead{(kpc)} & \colhead{} & \colhead{} & \colhead{} & \colhead{} & \colhead{}
}
\startdata
LMC & 80.8942 & -69.7561 & 0.05 & -18.1 & 9.3 & \nodata & 3.5 & 3.6 & 1.7 & \nodata & \citet{Skibba2012LMC} \\
\hspace{1em}SMC & 13.1580 & -72.8003 & 0.06 & -16.8 & 8.5 & 1.08 & \nodata & \nodata & \nodata & Y & \citet{Pace2024} \\
\hline
NGC~6822 & 296.2404 & -14.8031 & 0.46 & -15.2 & 8.1 & \nodata & 0.5 & 0.6 & 1.7 & \nodata & \citet{Zhang2021_NGC6822} \\
\hspace{1em} No Satellites \\
\hline
M33 & 23.4617 & 30.6603 & 0.84 & -18.8 & 9.7 & \nodata & 1.5 & 1.5 & 1.7 & \nodata & \citet{Corbelli2014} \\
\hspace{1em} No Satellites \\
\hline
NGC~3109 & 150.7769 & -26.1549 & 1.34 & -14.9 & 8.2 & \nodata & -0.3 & -0.1 & -1.2 & \nodata & \citetalias{McConnachie2012} \\
\hspace{1em}Antlia & 151.0171 & -27.3311 & 1.35 & -10.4 & 6.4 & 0.46 & \nodata & \nodata & \nodata & Y & \citetalias{McConnachie2012} \\
\hspace{1em}Antlia B & 147.2337 & -25.9900 & 1.29 & -9.7 & 6.2 & 0.27 & \nodata & \nodata & \nodata & Y & \citet{Sand2015} \\
\hline
NGC~300 & 13.7227 & -37.6842 & 2.00 & -18.4 & 9.2 & \nodata & 0.1 & 0.2 & 0.2 & \nodata & \nodata \\
\hspace{1em}Sculptor C & 14.4675 & -35.8523 & 2.04 & -9.1 & 5.7 & 0.36 & \nodata & \nodata & \nodata & Y & \nodata \\
\hline
NGC~55 & 3.7208 & -39.1966 & 2.34 & -18.5 & 9.7 & \nodata & 0.0 & 0.2 & 0.2 & \nodata & \citet{Kudritzki2016} \\
\hspace{1em}NGC55-dw1 & 3.8740 & -38.4190 & 2.20 & -8.0 & 5.2 & 2.20 & \nodata & \nodata & \nodata & Y & \citet{McNanna2024} \\
\hspace{1em}ESO294-010 & 6.6391 & -41.8561 & 2.03 & -11.3 & 6.4 & 0.25 & \nodata & \nodata & \nodata & Y & \citet{Medoff2025} \\
\hline
NGC~4214 & 183.9121 & 36.3275 & 3.04 & -17.5 & 8.8 & \nodata & 0.6 & 0.8 & -0.6 & \nodata & \citet{Dalcanton2009} \\
\hspace{1em}MADCASH-2 & 182.5281 & 35.4429 & 3.00 & -9.2 & 5.8 & 0.13 & \nodata & \nodata & \nodata & Y & \citet{Carlin2021} \\
\hspace{1em}DDO113 & 183.7412 & 36.2189 & 2.95 & -12.2 & 7.1 & 0.62 & \nodata & \nodata & \nodata & Y & \citet{Garling2020} \\
\hline
NGC~2403 & 114.2117 & 65.6022 & 3.19 & -19.1 & 9.7 & \nodata & 0.2 & 0.6 & 1.9 & \nodata & \citetalias{Karachentsev2013} \\
\hspace{1em}MADCASH-1 & 114.2140 & 65.6010 & 3.41 & -7.8 & 5.3 & 0.18 & \nodata & \nodata & \nodata & Y & \citet{Carlin2016,Carlin2024} \\
\hspace{1em}DDO044 & 113.5479 & 66.8797 & 2.96 & -12.9 & 7.3 & 0.74 & \nodata & \nodata & \nodata & Y & \citet{Karachentsev1999DDO044,Carlin2019} \\
\hline
NGC~3077 & 150.8375 & 68.7339 & 3.85 & -17.8 & 9.4 & \nodata & 2.3 & 2.4 & 1.9 & \nodata & \citet{Garling2021} \\
\hspace{1em} No Satellites \\
\hline
IC~2574 & 157.0933 & 68.4161 & 3.93 & -17.1 & 8.8 & \nodata & 1.5 & 1.7 & 1.9 & \nodata & \citet{Garling2021} \\
\hspace{1em} No Satellites \\
\hline
NGC~4449 & 187.0458 & 44.0936 & 4.02 & -18.4 & 9.5 & \nodata & 0.8 & 0.8 & 1.4 & \nodata & \citet{Sabbi2018} \\
\hspace{1em}LV J1228+4358 & 187.1867 & 43.9683 & 4.07 & -13.0 & 7.0 & 1.30 & \nodata & \nodata & \nodata & Y & \citet{Martinez-Delgado2012,Garling2021} \\
\hline
NGC~4236 & 184.1804 & 69.4656 & 4.44 & -18.2 & 9.4 & \nodata & -0.2 & 0.0 & 0.0 & \nodata & \citet{Garling2021} \\
\hspace{1em} No Satellites \\
\hline
NGC~5023 & 198.0496 & 44.0386 & 6.05 & -16.5 & 8.8 & \nodata & -0.9 & -0.3 & -1.1 & \nodata & \citetalias{Karachentsev2013} \\
\hspace{1em}dw1310+4358 & 197.7499 & 43.9802 & \nodata & -8.0 & 5.7 & 0.12 & \nodata & \nodata & \nodata & N & \citet{Carlsten2020} \\
\hspace{1em}dw1314+4420 & 198.6433 & 44.3342 & \nodata & -7.0 & 5.0 & 0.10 & \nodata & \nodata & \nodata & N & \citet{Carlsten2020} \\
\hline
NGC~1156 & 44.9267 & 25.2375 & 6.87 & -17.4 & 9.0 & \nodata & -1.5 & -1.2 & -1.3 & \nodata & \citetalias{Karachentsev2013} \\
\hspace{1em}NGC1156-dw1 & 45.0758 & 25.2489 & \nodata & -10.5 & 6.1 & \nodata & \nodata & \nodata & \nodata & N & \citetalias{Karachentsev2013} \\
\hspace{1em}NGC1156-dw2 & 45.1138 & 25.3051 & \nodata & -10.1 & 6.3 & \nodata & \nodata & \nodata & \nodata & N & \citetalias{Karachentsev2013} \\
\hspace{1em}dw0301+2446 & 45.3842 & 24.7832 & \nodata & -10.6 & 6.5 & \nodata & \nodata & \nodata & \nodata & N & \citet{Carlsten2020} \\
\hspace{1em}AGES J030039+254656 & 45.1625 & 25.7822 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & N & \citet{Minchin2010} \\
\hline
NGC~45 & 3.5162 & -23.1822 & 6.64 & -20.0 & 9.1 & \nodata & -1.0 & -0.9 & 0.2 & \nodata & \citet{Muller2020} \\
\hspace{1em} No Satellites \\
\hline
NGC~672 & 26.9717 & 27.4336 & 7.18 & -18.2 & 9.5 & \nodata & 0.2 & 0.3 & 0.2 & \nodata & \citetalias{Karachentsev2013} \\
\hspace{1em}IC1727 & 26.8745 & 27.3333 & 7.45 & -17.3 & 9.3 & 3.30 & \nodata & \nodata & \nodata & Y & \citetalias{Karachentsev2013} \\
\hspace{1em}NGC672-dwA & 26.8304 & 27.2548 & \nodata & -9.4 & 5.5 & 0.20 & \nodata & \nodata & \nodata & N & \citet{Davis2024} \\
\hline
NGC~24 & 2.4850 & -24.9633 & 7.31 & -20.3 & 9.2 & \nodata & 0.3 & 0.6 & 0.1 & \nodata & \citetalias{Karachentsev2013} \\
\hspace{1em}dw0009-25 & 2.4075 & -25.0492 & \nodata & -8.3 & 5.9 & 0.28 & \nodata & \nodata & \nodata & N & \citet{Muller2020} \\
\hspace{1em}dw0010-25 & 2.6592 & -25.3349 & \nodata & -11.6 & 6.7 & 1.05 & \nodata & \nodata & \nodata & N & \citet{Muller2020} \\
\hline
NGC~925 & 36.8167 & 33.5781 & 9.55 & -19.8 & 9.9 & \nodata & 1.0 & 1.1 & 0.5 & \nodata & \citetalias{Karachentsev2013} \\
\hspace{1em}d0226+3325 & 36.7200 & 33.4269 & \nodata & -12.0 & 7.0 & 1.50 & \nodata & \nodata & \nodata & N & \citet{PWE98,Davis2024} \\
\hline
NGC~4592 & 189.8279 & -0.5319 & 9.02 & -18.0 & 9.0 & \nodata & -0.4 & 0.1 & 1.2 & \nodata & \citet{Kim2020} \\
\hspace{1em}NGC4592-dw15 & 189.7053 & -0.5978 & 9.02 & -10.8 & 6.1 & 0.23 & \nodata & \nodata & \nodata & Y & \citet{Kim2022,CarlstenELVES2022} \\
\hspace{1em}NGC4592-dw16 & 189.7608 & -0.6650 & 9.02 & -13.2 & 7.2 & 0.74 & \nodata & \nodata & \nodata & Y & \citet{Kim2022,CarlstenELVES2022} \\
\hline
M96-DF6 & 161.7212 & 12.7426 & 10.20 & -13.4 & 7.6 & \nodata & 2.0 & 2.0 & 2.0 & \nodata & \citet{Cohen2018} \\
\hspace{1em}dw1046+1244& 161.6915 & 12.7499 & \nodata & -8.1 & 5.4 & 0.21 & \nodata & \nodata & \nodata & N & \citet{Muller2023} \\
\hline
\enddata
\tablecomments{This table presents a compilation of classical satellite candidates ($M_\star > 10^{5}\ M_\odot$) associated with dwarf galaxies ($M_\star <10^{10}\ M_\odot$) in the Local Volume ($<12\ \rm Mpc$) from the literature. For each system, the host galaxy is listed first, followed by its satellite candidates. We include key properties for both hosts and satellite candidates: Right Ascension and Declination (R.A. and Decl.), distance, $V$-band absolute magnitude ($M_V$), estimated stellar mass $\log M_\star$, and physical effective radius ($r_{\rm eff}$). For host galaxies, we also provide the tidal indices ($\Theta_1$, $\Theta_5$, $\Theta_j$) from \citet{Karachentsev2013}, which characterize their environment. Satellites that are confirmed with direct distances or radial velocities are marked as ``Y'' in the Conf. column. References for each object are provided in the final column. See Appendix \ref{sec:literature} for detailed descriptions of individual systems. }
\end{deluxetable*}
\end{longrotatetable}
